Some properties of catalog of (3, g) Hamiltonian bipartite graphs: orders, non-existence and infiniteness

The focus of this paper is on discussion of a catalog of a class of (3, g) graphs for even girth g. A (k, g) graph is a graph with regular degree k and girth g. This catalog is compared with other known lists of (3, g) graphs such as the enumerations of trivalent symmetric graphs and enumerations of trivalent vertex-transitive graphs, to conclude that this catalog has graphs for more orders than these lists. This catalag also specifies a list of orders, rotational symmetry and girth for which the class of (3, g) graphs do not exist. It is also shown that this catalog of graphs extends infinitely.

==> new_infinite_notes.tex <==


\begin{notation} \textbf{c(x)} \\
Given any node with label $x$ where $1 \le x \le 2m$, we denote the node to which the chord connects to node $x$ as $c(x)$.\\
If the HBG has D3 chord indices $d_1. d_2, ...., d_b$, symmetry factor $b$ and order $2m$, then 
if $x$ is odd, then $c(x)$ is defined as follows.\\
$i = x\ \%\ 2b$ \\
if($i = 0$) then $i = 2b$ \\
$c(x) = (h + d_{i})\ \%\ 2m$ \\
if $c(x) = 0$ then $c(x) = 2m$\\
If $x$ is even, then $c(x)$ is defined as an odd number $y$, where $c(y) = x$.
\end{notation}

\begin{notation} \textbf{p(x)} \\
Given any node with label $x$ where $1 \le x \le 2m$, we denote the previous node p(x) as 
$p(x) = (x - 1) \ \%\ 2m$ \\
if $p(x) = 0$ then $p(x) = 2m$
\end{notation}

\begin{notation} \textbf{n(x)} \\
Given any node with label $x$ where $1 \le x \le 2m$, we denote the next node n(x) as 
$n(x) = (x + 1) \ \%\ 2m$ \\
if $p(x) = 0$ then $p(x) = 2m$
\end{notation}



\begin{note} \textbf{Traversals on HBGs} \\
Let us examine breadth first traversals on a HBG with D3 chord indices $d_1. d_2, ...., d_b$, symmetry factor $b$ and order $2m$.\\
Without loss of generality we consider breadth first traversals starting at nodes $1, 2, ...., 2b$ (due to rotational symmetry). Let us consider all traversals starting at node $h$ where $1 \le h \le 2b$, as tree with the following structure.\\
Starting from depth $0$, where we have one node with label $h$, we visualize a tree using the following rules.
\begin{itemize}
\item Each node $x$ has successor nodes $c(x)$ if parent node $y$ of $x$ then $x \ne c(y)$, and $p(x)$ if parent node of $x$ is not $n(x)$ and $n(x)$ if parent node of $x$ is not $p(x)$.
\item \textbf{Repeated label criterion} We terminate the tree at particular depth $k$, if any of the nodes at depth $k$ have the same label as another other node of the tree.
\end{itemize}

\begin{example}
For simplicity, let us consider symmetry factor $1$, D3 chord index $5$, and order 12.\\
Depth 1: 1 has successors 12, 2, and 6 \\
Depth 2: 12 has sucessors 11 and 7\\
2 has sucessors 3 and 9\\
6 has sucessors 7, 5\\ We stop here since 7 is a repeated label.
We now find a cycle $7 \to 6 \to 1 \to 7$ which is of length $4$.
\end{example}

\begin{example}
For simplicity, let us consider symmetry factor $1$, D3 chord index $5$, and order 14.\\
Depth 1: 1 has successors 14, 2, and 6 \\
Depth 2: 14 has sucessors 13 and 9\\
2 has sucessors 3 and 11\\
6 has sucessors 7, 5\\
Depth 2: 13 has successors 12 and 4\\
7 has successors 8, 12\\ We stop here since 12 is a repeated label.
We now find a cycle $12 \to 7 \to 6 \to 1 \to 14 \to 13 \to 12$ which is of length $6$.
\end{example}

\begin{example}
 Generalizing the above idea, for a HBG symmetry factor $1$, D3 chord index $l = 5$ with an arbitrary order $2m$ where $2m \ge 14$,
 Depth 1: 1 has successors $2m$, 2, and $l + 1$ \\
Depth 2: $2m$ has sucessors $2m - 1$ and $2m - l$\\
2 has sucessors 3 and $2m - 3$\\
$l + 1$ has sucessors $l + 2$, $l$\\
Depth 3: $2m - 1$ has successors $2m - 2$ and $2m - 1 + l$\\
$l + 2$ has successors $l + 3$, $2 m - 2$\\ We stop here since $2 m - 2$ is a repeated label.
We now find a cycle $2m - 2 \to 2m-7 \to 2m - 8 \to 1 \to 2m \to 2m - 1 \to 2m - 2$ which is of length $6$.
\end{example}
  


\end{note}


%\begin{notation} \textbf{Parametric breadth first traversal} \\

%\end{notation}

%\begin{note} \textbf{When do we say that two sets of traversal trees are the same?} \\
%If two HBGs $G_a$ and $G_b$ with symmetry factor $b$ and orders $2kp$ and $2kq$ have the identical traversal trees for nodes $1, 3, ..., 2b-1$ as a function of order, then $G_a$ and $G_b$ have the same girth. In this case, we also say that their traversal trees as a function of order are the same.
%\end{note}



\begin{theorem}
Given D3 chord indices $d_1, d_2, ...., d_b$ with symmetry factor $b$, there exists a threshold $2bk$, such that HBGs with D3 chord indices $d_1. d_2, ...., d_b$ with symmetry factor $b$ and order $2b (k + i)$ have the same girth, where $i = 0, 1, 2, ...$.
\end{theorem}
\begin{proof}
Let us consider a HBG with order $2m_1$, symmetry factor $b$, with D3 chord indices $d_1. d_2, ...., d_b$. Let us consider the Breadth first traversal trees starting at nodes $1, 3, ..., 2b-1$ as a function of order $2m_1$.\\
Similarly, let us consider a HBG with order $2m_2$, symmetry factor $b$, with D3 chord indices $d_1. d_2, ...., d_b$. Let us consider the Breadth first traversal trees starting at nodes $1, 3, ..., 2b-1$ as a function of order $2m_2$.\\


It is clear that there exists a threshold $2m = 2bk$, such that all node labels in tree are distinct, until the first repeated label corresponding to a cycle is found, which means that all these parametric traversal trees as a function of order are identical, for orders $2b (k + i)$, where $i = 0, 1, 2, ...$, which is turn means that the girth of the HBGs beyond the threshold is the same.
\end{proof}
